Computational LEGO Technic Design

We introduce a method to automatically compute LEGO Technic models from user input sketches, optionally with motion annotations. The generated models resemble the input sketches with coherently-connected bricks and simple layouts, while respecting the intended symmetry and mechanical properties expressed in the inputs. This complex computational assembly problem involves an immense search space, and a much richer brick set and connection mechanisms than regular LEGO. To address it, we first comprehensively model the brick properties and connection mechanisms, then formulate the construction requirements into an objective function, accounting for faithfulness to input sketch, model simplicity, and structural integrity. Next, we model the problem as a sketch cover, where we iteratively refine a random initial layout to cover the input sketch, while guided by the objective. At last, we provide a working system to analyze the balance, stress, and assemblability of the generated model. To evaluate our method, we compared it with four baselines and professional designs by a LEGO expert, demonstrating the superiority of our automatic designs. Also, we recruited several users to try our system, employed it to create models of varying forms and complexities, and physically built most of them.

==> construction.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Construction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Two-Stage Framework: Stage 2}
\label{sec:our_framework2}

Before we present the overall procedure in the second stage of our framework in Section~\ref{ssec:main_procedure}, we first present how we modify a beam layout (Section~\ref{ssec:update_operator}) and connect adjacent beams (Section~\ref{ssec:connecting_beams}).
%After that, we will present the further analysis on the generated model (Section~\ref{ssec:main_procedure}).

%Before we present the overall procedure in the second stage of our framework in Section~\ref{ssec:main_procedure}, we first %present the operator to modify the beam layout (Section~\ref{ssec:update_operator}) and the procedure to connect beams %(Section~\ref{ssec:connecting_beams}).
%After that, we will present the further analysis on the generated model (Section~\ref{ssec:main_procedure}).

%This section presents the second stage of our annealing framework.
%Before we present the overall procedure, we first present the operator for modifying the beam layout %(Section~\ref{ssec:update_operator}) and how we connect beams through the various connection mechanisms %(Section~\ref{ssec:connecting_beams}).
%After that, we present the overall procedure in our framework for arranging beams and iteratively refining the beam layout %(Section~\ref{ssec:main_procedure}), and then present our analysis on the generated model and the assembly of the physical %Technic model (Section~\ref{ssec:postprocessing}).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Operator to Modify the Beam layout}
\label{ssec:update_operator}

%An important element in stage 2 of our framework is the operator to modify the beam layout.
%
To design the operator to modify the beam layout, we first have to keep in mind that the operator must be efficient, due to heavy usage in the annealing process.
%
Second, even the operator is local, successively applying it should lead to global modifications that improve the beam layout.
Lastly, the beam layout should eventually converge at the end of the annealing process.

\vspace*{-5pt}
\paragraph{Procedure}
The operator we designed to meet the goals has five steps as illustrated in Figure~\ref{fig:operator}:
(i) we randomly pick a covered edge in the guiding graph;
(ii) we remove all the beams that associate with the edge, including also those that stop at the edge endpoints;
(iii) we lookup all possible beam placements that can cover the ``uncovered'' edge(s) resulted from the beam removal, and compute the selection probability for each candidate placement: the number of uncovered edges that the candidate beam covers normalized by the total number of uncovered edges over all the candidate beams;
(iv) we randomly select a candidate placement based on the probability and add the beam in a layer that favors a more compact layering (see Eq.~\eqref{eq:cpt}); and
(v) we repeat steps (iii) and (iv) until we cover all the uncovered edges, or until the nodes (beam holes) in the remaining uncovered edges are occupied by some other beams in the existing layout; see Figure~\ref{fig:example_conn_cover} (middle) for an example of such a situation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
  \centering
  \includegraphics[width=8.35cm]{images/operator.png}
  \vspace*{-1mm}
  \caption{Our operator to modify the beam layout has five steps altogether; please see Section~\ref{ssec:update_operator} for the procedural details.  \legoclaim}
%  \caption{The procedure in our operator to modify a beam layout; please see Section~\ref{ssec:update_operator} for the procedural details.}
  \label{fig:operator}
  \vspace*{-2mm}
\end{figure}


\vspace*{-5pt}
\paragraph{Discussion}
%Before we come up with the above procedure
Before we settle the above procedure, we have explored many alternative designs.
For example, we tried to choose candidate placements with equal probability in step (iii) and to remove only the beams that cover (but not touch) the selected edge in step (ii).
%
For the former case, the annealing process becomes too slow, even for simple models, while for the latter case, the modification becomes so small that we can hardly find any good solution.
% that minimizes the objective function.
%
On the other hand, we tried to remove more nearby beams in step (ii), but the modification becomes so large that the annealing process is hard to converge.
%
Furthermore, we tried to divide our operator into two (one to remove beams and the other to add beams) and apply them at random; however, the intermediate beam layout becomes mostly incomplete, so the annealing process is also hard to converge.
%
%However, if we randomly apply these two operators rather than one immediately after the other, the intermediate beam layout are mostly incomplete, so the annealing process is also hard to converge.

% discussion of our operator
%When adding new beams, instead of directly forbidden putting an overlapping beam, we allow adding beams with overlap with a certain probability, 
%such that we can flexibility achieve different objectives(such as locally objective) using the same operator.
% operator with same chosen probability
%In our initial attempts, we beam candidates with the same probability, as a result, chosen beams have high chances to be overlapped, making the search process slow to find a simple structure. 
% remove one beam, only remove the edge, or remove larger region.
%Besides, we also tried to remove one beam or only remove beams passing through the chosen edge, which updates a smaller local region in each iteration. 
%However, the search is hard to converge to a simple structure or even a feasible solution, since small locally update is hard to achieve a good solution for the entire model.
%On the other hand, we also tried to remove a larger region(e.g. remove one-ring beam neighbors also), as a result, the region is so large that makes single iteration contains a huge decision space.
% multi-operator in the model
%Another direction of the simulated annealing algorithm is to design several operators, such that these operators are applied alternatively to achieves the final objectives.
%We experiment with this idea by separate our operator into two "removal" and "adding" operator and then choose the two operator in the same probability. 
%However, beam layout may be incomplete in each iteration, we add another term in our objective function to evaluate the model completeness to guide the search.
%However, we find it hard to converge to a complete model in the end, although we can occasionally get a complete model by tune the weight of completeness term for different input.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Connecting beams}
\label{ssec:connecting_beams}

Another important element in our framework is the method, or procedure, to find connection mechanisms (see Figure~\ref{fig:brickset_and_connections} (right)) to connect adjacent beams in a beam layout.
Particularly, we need to connect beams for evaluating the connection coherence in the objective function during the annealing process, and in the end, we need to connect beams to form a complete model.

%, particularly for beams that have different orientations.
%
Procedure-wise, given the current beam layout, we first identify edges in the guiding graph that are not covered by any beam in the layout, and group together the adjacent uncovered edges; see the leftmost column in Figure~\ref{fig:running_connection}.
%
Then, we use a distance threshold of $\sqrt{3}$ units to identify beam holes around each group; see the highlighted beam holes in the middle column of Figure~\ref{fig:running_connection}.
Now, our goal is to find connection mechanisms that can connect these identified beam holes between beams around the uncovered edges.

In general, beam connections are not always one-to-one, i.e., two beams joined by a single mechanism; see Figure~\ref{fig:running_connection} (top row case).
%
First, some connection mechanisms can join three or more beams together, e.g., the T-shaped mechanism in Figure~\ref{fig:brickset_and_connections} (right) and the middle row case in Figure~\ref{fig:running_connection}, where the L-shaped mechanism joins the three beams altogether.
%
Second, we sometimes need more than one connection mechanisms to join the beams around the uncovered edges, e.g., see the bottom row case in Figure~\ref{fig:running_connection}, where we use two mechanisms to connect the three beams in the example.

To connect a set of adjacent beams, we first find all feasible connection mechanisms that can join beam holes of different beams.
In case there are three or more adjacent beams in the set,
%around the group of uncovered edges, 
we further find subsets of the feasible connection mechanisms that can connect all the beams.
%
To choose between the connection mechanisms, we have four considerations:
%
(i) the chosen mechanisms should not collide with the existing beams in the layout, and if we use two or more mechanisms, the bricks in the mechanisms should not collide with one another;
(ii) we want minimal overall pin-head ratio to aim for simpler connections;
(iii) we avoid connection mechanisms whose connecting bricks (pins, connectors, and axles) go below the ground plane; see Figure~\ref{fig:conn_consider} (top); and 
(iv) for aesthetics, we can manually mark undesirable mechanisms for our tool to avoid, e.g., connecting bricks that extend outward; see Figure~\ref{fig:conn_consider} (bottom).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
  \centering
  \includegraphics[width=8.35cm]{images/running_connection.png}
  \vspace*{-1mm}
  \caption{The procedure to find connection mechanisms (see Figure~\ref{fig:brickset_and_connections} (right)) to join adjacent beams; see Section~\ref{ssec:connecting_beams} for the details.  \legoclaim}
  \label{fig:running_connection}
  \vspace*{-2mm}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stage 2: Overall Procedure}
\label{ssec:main_procedure}

After we present the operator to modify the beam layout and the method to connect beams, we are ready to present the overall procedure in stage 2 of our simulated-annealing-based framework.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Layout initialization.}
Our procedure starts by repeating the following steps to initialize a beam layout:
%
randomly pick an uncovered edge in the guiding graph (all edges are uncovered initially) and then randomly select and add a beam to cover the edge, similar to steps (iii)-(v) in the layout modification operator (see Section~\ref{ssec:update_operator}).
%
However, unlike the operator, we select candidate beams with equal probability to deliberately generate a more random initial layout (see Figure~\ref{fig:overview}(c) for an example), since a more random layout helps the simulated-annealing process avoid local minima.
%
% instead of greedily generating the initial layout to minimize the objective function, we deliberately generate a more random layout, so that the search process will not easily stuck at local minima.

%\phil{TODO: (i) how (the procedure to initialize) and (ii) discuss why this is sufficient already}
%Our initialization algorithm start from a guiding graph and an empty beam set $\mathcal{B}$.
%Then, the algorithm proceed as follows:
%\begin{itemize}
%	\item[(i)]
%	Randomly pick an uncovered edge $e$ in the guiding graph;
%	\item[(ii)] 
%	Find all possible beam placements that pass through edge $e$;
%	\item [(iii)]
%	We then randomly select a candidate beam $b$ with random layer number, add $b$ and its symmetry beams to $\mathcal{B}$; %and
%	\item [(iv)]
%	We repeat step (i), (ii), and (iii) until all the nodes in the guiding graph have a associate beam.
%\end{itemize}
%After the above procedure, we got $\mathcal{B}$ as a messy layout, see Figure. \ref{fig:overview} middle left for an initial %layout for our {\sc crossbow} model.
%%discussion
%Note that instead of creating a better initial layout using other strategies such as greedy, we deliberately add some random %variations to avoid the searching process start from a local minimum position, which may make the search process stuck in a local %region.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
  \centering
  \includegraphics[width=8.35cm]{images/conn_consider.png}
  \vspace*{-1mm}
  \caption{We avoid connection mechanisms whose bricks go below the model's ground plane (top) or extend outward (bottom).  \legoclaim}
  \label{fig:conn_consider}
  \vspace*{-2mm}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Objective function.}
We guide the beam layout refinement by minimizing the objective function $\mathcal{F}$ presented in Section~\ref{ssec:obj}.
In our implementation, we adopt the components in the objective function (see Eq.~\eqref{eq:obj}) for the simulated annealing process as follows:
%
\begin{itemize}

%1  w_\text{dev}
%2  w_\text{cpt}
%3  w_\text{sym}
%4  w_\text{tbl}
%5  w_\text{phr}
%6  w_\text{col}
%7  w_\text{gap}
%8  w_\text{coh}
%9  w_\text{rgd}

\vspace*{-1mm}
\item
First of all, to balance the various components in the objective, we empirically set $w_\text{cpt}$, $w_\text{sym}$, $w_\text{phr}$, $w_\text{col}$, $w_\text{gap}$, and $w_\text{coh}$ as $1$, $30$, $10$, $30$, $100$, and $50$, respectively, and adjust $w_\text{dev}$, $w_\text{tbl}$, and $w_\text{rgd}$ based on user preference.
In practice, we set $\{ w_\text{dev}, w_\text{tbl}, w_\text{rgd} \}$ as $\{100,0,0\}$ to aim for high faithfulness to the input sketch, as $\{0,100,0\}$ to aim for model simplicity, and as $\{100,0,100\}$ or $\{0,100,100\}$ to additionally aim for rigid connections.
%
%First of all, the requirements modeled by various components in the objective may contradict one another, for example, a simple layout with minimized total beam length (see Eq.~\eqref{eq:simplicity}) contradicts the rigidity requirement, which encourages adjacent beams to connect with two or more beam holes to achieve more rigid connections (see Eq.~\eqref{eq:rgd}).
%
%In our implementation, we fix the weights $w_2$, $w_3$, $w_5$, $w_6$, $w_7$, and $w_8$ as $1$, $30$, $10$, $30$, $100$, and $50$, respectively, while we adjust $w_1$, $w_4$, and $w_9$ based on the user preference.
%
%In practice, we set $\{ w_1, w_4, w_9 \}$ as $\{100,0,0\}$ to aim for high faithfulness to the input sketch ($\mathcal{F}_f$),
%as $\{0,100,0\}$ to aim for the simplest beam layout ($\mathcal{F}_s$), and 
%as $\{100,0,100\}$ or $\{0,100,100\}$ to additionally aim for rigid connections.

\vspace*{-1mm}
\item
Second, the beam layout starts to be highly random, where most beams will not stay until the end.
%
Hence, it is not useful to evaluate the collision ($\mathcal{F}_\text{col}$) and connection coherence ($\mathcal{F}_\text{coh}$) terms, when the layout is not yet stable.
%
Particularly, evaluating $\mathcal{F}_\text{coh}$ involves relatively more computation than the other terms in the objective, since we need to find connection mechanisms between adjacent beams (see Section~\ref{ssec:connecting_beams}).
%
Hence, we define $\mathcal{F}^o$ as a simplified version of $\mathcal{F}$ (see Eq.~\eqref{eq:obj}) without $\mathcal{F}_\text{col}$ and $\mathcal{F}_\text{coh}$, and use $\mathcal{F}^o$ instead of $\mathcal{F}$ in early annealing process.

\vspace*{-1mm}
\item
Lastly, since the layout modification operator is local, we actually update the objective function value based on the local changes in the layout every time we modify the layout.

\end{itemize}


%\phil{TODO:
%(i) we aim to minimize $\mathcal{F}$ (see Eq.~\eqref{eq:obj}) in order to create a beam layout for faithfulness to the input %sketch, structural simplicity, and structural integrity;
%(ii) weights on different terms in the objective functions... how to tune and why?
%(iii) for efficiency concern, we do not explicitly create beam connections (since the beam layout ...) over the annealing %process, some 
%then, define $\mathcal{F}^0$ and $\mathcal{F}^1$, which is the incomplete version and the complete version
%(iv) moreover, since the operator only modifies the local beam layout, we in fact locally update the objective function for %higher efficiency}

% minimization
%We optimize the beam layout by minimizing all the terms we mentioned in Section.\ref{sec:modeling}.
%% trade-off
%However, minimize one objective may violate another, so we can not achieve multiple optimal objective in a same beam layout. For %example, a simple layout which minimized the number of beam holes will contradict the rigidity objective, which need more than %one hole to for a rigid local connection.
%In Sec~\ref{sec:modeling}, most terms are served as penalty except for $\mathcal{F}_\text{dev}$ $\mathcal{F}_s$, and %$\mathcal{F}_\text{rgd}$.
%So impractically, we set $w2$,$w3$,$w6$,$w7$,$w8$ as $(?,?,?,?,?)$(check from code after I get back ), and leave the necessary %trade-off between $w_1$,$w_4$,$w_5$, and $w_9$ to user to indicate their preference.

% connectness evaluation -> slow
%Third, the algorithm to evaluation connection coherency in Eq.~\eqref{eq:cohr} contains procedure which require exhaustive search %for a local region, so it often takes more time than other terms. 
%Besides, we observe that at high temperatures, a simulated annealing algorithm accepts virtually all inferior steps and resembles %a random search, making the beams distribute sparsely and disordered. In this case, evaluating connectedness not much efficient %to guide the search, since nearly all the intermediate layout is not coherently connected.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% pseudo-code
\begin{algorithm} % enter the algorithm environment
\caption{Overall Procedure in Stage 2} % give the algorithm a caption
\label{alg:SA} % and a label for \ref{} commands later in the document
\begin{algorithmic} % enter the algorithmic environment
\REQUIRE $T_\text{max}$, $T_\text{min}$, $T_\text{mid}$, $r$, and Guiding graph $\mathcal{G}$
\STATE $\mathcal{B}_\text{current} = \ \text{initialize}\_\text{layout}(\mathcal{G})$
\hspace*{2mm}     // initialize the beam layout
\STATE $T \hspace*{8.25mm} = \ T_\text{max}$
\hspace*{21.25mm}  // initialize temperature T
\STATE $\mathcal{B}_\text{best} \hspace*{3.4mm} = \ \mathcal{B}_\text{current}$
\hspace*{17.25mm} // initialize the best layout
\STATE $\mathcal{F}_\text{obj} \hspace*{4.75mm} = \ \mathcal{F}^o$
\hspace*{23.15mm}  // set objective func. in use
\WHILE{ \ $T \ > \ T_\text{min}$ \ }
	\IF{ \ $T \ < \ T_\text{mid}$ \ }
		\STATE $\mathcal{F}_\text{obj} \ = \ \mathcal{F}$
		\hspace*{22.35mm} // switch to full obj. func.
	\ENDIF
	\STATE $\mathcal{B}_\text{new} = \ \text{modify}(\mathcal{B}_\text{current})$
	\hspace*{6mm} // apply operator in Sec.~6.1
	\STATE $\Delta \ \hspace*{4.05mm} = \ \mathcal{F}_\text{obj}( \mathcal{B}_\text{new} ) \ - \ \mathcal{F}_\text{obj}( \mathcal{B}_\text{current} )$
	\IF{ \ $\exp(-\Delta / T ) \ > \ \text{rand}(0,1) $ \ }
	\STATE $\mathcal{B}_\text{current} \ = \  \mathcal{B}_\text{new} $
	\hspace*{13.35mm} // accept the change
	\IF{ \ $\mathcal{F}_\text{obj}(\mathcal{B}_\text{current}) \ > \ \mathcal{F}_\text{obj}(\mathcal{B}_\text{best}) $ \ }
	\STATE 	$\mathcal{B}_\text{best} \ = \ \mathcal{B}_\text{current} $
	\hspace*{10.4mm} // update best layout
	\ENDIF
	\ENDIF
	\STATE $T \ = \ T*r$
	\hspace*{25.55mm} // update temperature $T$
	\ENDWHILE
	\STATE \textbf{return} \hspace*{1mm} $\mathcal{B}_\text{best}$
\end{algorithmic}
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Overall procedure}
We adopt the simulated annealing model by Cagan et al.~\shortcite{cagan1998simulated} to regulate the solution search process.
%
Our model has four parameters: $T_\text{max} > T_\text{mid} > T_\text{min}$ and $r$, which denote the starting temperature, middle cutoff temperature, ending temperature, and cooling rate, respectively.
We empirically set $T_\text{max}$ as $2$$\times$$10^3$, $T_\text{mid}$ as $10$, $T_\text{min}$ as $10^{-4}$, and $r$ (which trades off model quality and running time) as $0.999$ for simple models and as $0.99997$ for large and complex models.
%
In the annealing process, we use $\mathcal{F}^o$ when current temperature $T \geq T_\text{mid}$, and switch to use $\mathcal{F}$ when $T < T_\text{mid}$.
%
%Another important parameter is the cooling rate $r$ for trading off between the model quality and running time; we set $r$ as $0.999$ for simple models and as $0.99997$ for large and complex models.
%
Algorithm~\ref{alg:SA} summarizes the overall procedure.
%
%After initializing the beam layout and various parameters, we enter the main loop, which iteratively modifies the current beam layout $\mathcal{B}_\text{current}$ using the layout modification operator (denoted as modify()).
%
%In each iteration, we compute the change in the objective value (denoted as $\Delta$) after the layout modification, and accept the modification if $e^{-\Delta/T}$ is greater than a uniformly-distributed random value between zero and one, where $T$ is the current temperature in the annealing process.
%
%Lastly, when $T$ drops below $T_\text{min}$, the annealing process ends and returns the best beam layout $\mathcal{B}_\text{best}$ as the output.

Recalling that due to the immense search space, we first estimate the beam orientation in our framework.
%
However, the estimated orientations may not be perfect all the time.
%
Hence, when the beam layout becomes stable, the layout modification operator will try different valid beam orientations (see the constraints in Section~\ref{ssec:beam_orient}) when adding beams.
%
One typical example is the two pontoons on the bottom of {\sc airplane}: the estimated orientation of the pontoon beams is upward (see Figure~\ref{fig:optimize_SA} (right)) but re-orientating them allows simpler connections (see Figure~\ref{fig:teaser}) that minimize the objective.

%Recalling that we have four sub-problems when arranging beams to build Technic models.
%Among them, we first estimate the beam orientation based on a heuristic (see Section~\ref{ssec:beam_orient}), since addressing the four sub-problems altogether involves a tremendously large search space, which makes the overall problem hard to solve.
%
%However, we found that the estimated beam orientations may not be perfect all the time.
%Hence, when the beam layout become stabilized, we allow the layout modification operator to try different beam orientations (as long as the beam is still parallel to the associated sketch line) when adding beams, so that we may further improve the objective function.
%
%One typical example is the two pontoons on the bottom of the {\sc plane} model.
%The estimated orientation of the pontoon beams is upward (see Figure~\ref{fig:optimize_SA} (right)), but re-orientating the beams can allow simpler connection mechanisms (see Figure~\ref{fig:teaser}), thus further minimizing the objective function value.

%After the annealing procedure, output beams will have the same orientation with what we estimated in %Section.~\ref{ssec:beam_orient}.
%However, some line-shaped component may get a better connection by rotating along its central axis.
%To further improve, we try two different orthogonal orientation for each line-shaped component, and then choose one orientation %that could make simpler and coherent connection.
%%See the difference between the pink line-shaped component in bottom Figure~\ref{fig:plane_components} and the corresponding %position in the final model in Figure~\ref{fig:teaser} for example.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Discussion}
Besides the exponential annealing schedule we employed, we have tried several alternatives: linear, logarithmic, and optimum (see~\cite{nourani1998comparison}), as well as an adaptive one, which is the thermodynamic schedule in~\cite{de2003placement}.
However, we found no obvious improvements in results and running time; we think this is because the search space is discrete rather than continuous, where feasible solutions are not close to one another.
%
Moreover, we extended Algorithm~\ref{alg:SA} to be a population-based simulated annealing search~\cite{van2007population} by finding $N$ instead of one solutions in each iteration and keeping the best $K$ of them for generating the candidates in the next iteration (we set $N$ = 20 and $K$ = 4).
However, we found that the solution quality improves only slightly and the running time increases a lot, so we just use $N=K=1$ when producing our results.

%In addition, we have tried a population-based simulated annealing search method~\cite{van2007population}, where we first %independently initialize $N$ different random layouts, and in each iteration, pick the $k$ best layouts to continue their %executions, and restart the remaining $N-k$ layouts from the best solution found so far, where $N$ and $k$ are set as 20 and 4, %respectively.
%While the quality of the solutions improves slightly, the method requires much longer running time; see Section~\ref{sec:results} for comparison results.
%This proves our initialization algorithm provides a \phil{what do you mean by high?} starting searching point with high objective value, as a result, the search process do not easily to stuck in local minimum.

%Lastly, we have also tried metaheuristics and use a swamp to solve the problem.
%Particularly, we implemented an ant colony optimization method~\cite{dorigo1999ant}, where each move represents the addition of a new beam, so a model construction is represented by a sequence of moves started from an empty layout.
%
%Ideally, the optimization should converge to a near-shortest path, representing a simple beam layout, but we found the method can hardly converge to even a feasible layout, due to the exceptionally ``long path'' and huge search space incurred in the problem.
%\TODO{show experiments and real parameter setting}

% annealing schedule
%Ideally, a simulated annealing model can be further accelerated by carefully select a suitable annealing schedule.
%Except for exponential annealing schedule we used in our algorithm, we have attempted to implement several other predetermined %annealing schedules such as linear, logarithmic and optimum schedule as discussed in ~\cite{nourani1998comparison}, and adaptive %annealing schedule such at thermodynamic in ~\cite{de2003placement}. 
%However, the strategies did not improve the results nor the time. It is particularly challenging in the parameter setting, given %the fact that the search space is discrete and less connected.

% population
%Typically, due the fact that SA is a solo-searcher, its final solution quality may depends on the starting point.
%We experiment our algorithm stableness by implementing a population based SA search in ~\cite{van2007population}, where each %solution instances are initialized into different beam layout using our layout initialization algorithm.
%Since our initialization algorithm provides a high starting point, the search process can jump over hills to avoid stuck in local %minimum in the earlier process.
%As a result, the solution quality only improved slightly, while the running time is several times longer.
%See our experiments in Section. \ref{sec:result}(\TODO{show experiments}).

% swarm intellengence->, ant colony, particle swarm
%Another important family in metaheuristic algorithm is to use the behavior of swarms to solve the problem.
% ant colony
%We first implemented an ant colony optimization process, in which every move representing placing a new beam, and a set of moves %forms a path from empty beam set to a final construction.
%During the searching process, each ant will leave pheromone to indicate the shortest path(to a low-objective solution) they %found.
%Ideally, as time goes by, the pheromone content on the path leading to a low-objective solution will increase.
%However, the process can hardly converge to a feasible beam layout due to the very "long path" and vast variations from am empty %set to the final construction.

% particle swarm
% XH : TODO: try to complete here after the experiment



\input{postprocessing}



==> method.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Related works
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Method}
\label{sec:method}

\subsection{Single Plane Legolization}
This subprogram aim to generate assembly for one plane.
\par The input is a 2D graph generated by the user sketch, output is the assembly model using beams and pins.
\par To generate the assembly for one plane, we have the following steps.
\begin{itemize}
	\item Graph Clustering
	\item Generate Grid Base Vector
	\item Fit Grid Point
	\item Fit Non-Grid Point
	\item Merge co-linear Beams
	\item Layering Arrangement
\end{itemize}
\par TODO:List Requirements for Single Plane Legolization

\subsubsection{Graph Clustering}
\par Since most of the human-designed Technic Series are based on grid. We hope to fit it into grid. But usually the whole assembly model contains several sub-component, each sub-component have it's own grid system. So the first step of generate a single plane assembly is to clustering(or group) the input graph into several group, and for each group, we can generate its grid system later.
\par Affinity Matrix: 
$$A(i,j) = connect(l_i,l_j)\ ?\ \frac{\pi}{4}|arcos( |\frac{\overrightarrow{l_i} \cdot \overrightarrow{l_j}}{|\overrightarrow{l_i}|\cdot|\overrightarrow{l_j}|}| )- \frac{\pi}{4} | : 0 $$
\par TODO: detail:why Spectrul Clustering. etc.

\subsubsection{Generate Grid Base Vector}
\par After the first clustering step, we have several sub-graphs. In this step, we need to generate grid that fit each point as closely as possible. To represent the gird, we generate the base vector based on the orientation of every lines.
\par 
\par TODO: generate base vector for grid,  give the evaluation function etc.

\subsubsection{Fit Grid Point}
\par If the group satisfy the grid configuration, our next goal is to put each graph point into appropriate gird point. At the same time, satisfy the following criterial.
\begin{itemize}
	\item Each Beam(Bar,line) is a multiply of the length of a hole(20 lego unit).
	\item The shape should be as close as possible to the input user sketch.
\end{itemize}
\par Method: For each graph point, we generated 9 condidate closest point on grid. And try all the combination of all candidate point, find the feasible result which have the minimum score of the evaluation function.
\par Since we will try all the combinations of each point, so the calculation time is so important. The average number of nodes for a subgraph is 6, So the average trying numbers is $9^6$
\par Evaluation Function:We denote the $i_{th}$ point as $O_i$current candidate point on point $i$ as $P_i$. Then the evaluation function is $$\sum_{i=0}^{n-1}|Q_i-P_i|$$. After trying all combinations, the left thing is to find the result with minimal score.

\par TODO:give evaluation function(how close between the sketch and the assembly model), analyze the possible solution.

\subsubsection{Fit Non-Grid Point}
\par However, our user may not always give a grid-based input. So we should judge whether the graph satisfy the grid-shape configuration.
\par For Non-Grid graph, we also hold the two criterial above. But the Method are diffrent.
\par Method: Generate random point for each point in a roundness area. And expect each line become an multiply of 20.
\par If we just generate random number for each point, and expect them all satisfy the conditions at the same time. The possibility may be very small. So our algrithm choose to fit the point 3 by 3.

\subsubsection{Merge co-linear Beams}
\par For each point, we find its adjacent lines. And calculate whether two of them are co-linear, which means the two co-linear beams can be replaced by a long single beam.
THRESHOLD:
$$arcos(|\frac{\overrightarrow{l_1}\cdot\overrightarrow{l_2}}{|\overrightarrow{l_1}| \cdot |\overrightarrow{l_2}|}|)<\frac{\pi}{180}$$
\par TODO: give the evaluation function. And give adjustment strategy when it's slightly not co-linear.

\subsubsection{Layering Arrangement}
\par When we have the 2D graph in x-y plane, next stage is to generate the 2.5D model, which means layer each beam in z-direction.
\par We have the following criteria.
\begin{itemize}
	\item adjacent beams can not collide(at the same layer) \&\& can not be seperated.
	\item Minimize the number of layers.
\end{itemize}
Try all possible combinations, remove the symmetry configurations etc.

\par TODO: judgement algrithm, collision detection etc.


\par Notice: do not do Rigid analysis now, do it latere. Maybe not rigid for a single plane, but rigid for the whole structure.


\subsection{Plane Connection Algorithm}
Here will be an algorithm to use connect patterns to connect each plane, including changing the orientations of the beams.

Cite something for compilation...~\cite{song2016}


==> method_draft.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Modeling
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Modeling}
\label{sec:modeling_TMP}

\subsection{Single Plane Legolization}
This subprogram aim to generate assembly for one plane.
\par The input is a 2D graph generated by the user sketch, output is the assembly model using beams and pins.
\par To generate the assembly for one plane, we have the following steps.
\begin{itemize}
	\item Graph Clustering
	\item Generate Grid Base Vector
	\item Fit Grid Point
	\item Fit Non-Grid Point
	\item Merge co-linear Beams
	\item Layering Arrangement
\end{itemize}
\par TODO:List Requirements for Single Plane Legolization

\subsubsection{Graph Clustering}
\par Since most of the human-designed Technic Series are based on grid. We hope to fit it into grid. But usually the whole assembly model contains several sub-component, each sub-component have it's own grid system. So the first step of generate a single plane assembly is to clustering(or group) the input graph into several group, and for each group, we can generate its grid system later.
\par Affinity Matrix: 
$$A(i,j) = connect(l_i,l_j)\ ?\ \frac{\pi}{4}|arcos( |\frac{\overrightarrow{l_i} \cdot \overrightarrow{l_j}}{|\overrightarrow{l_i}|\cdot|\overrightarrow{l_j}|}| )- \frac{\pi}{4} | : 0 $$
\par TODO: detail:why Spectrul Clustering. etc.

\subsubsection{Generate Grid Base Vector}
\par After the first clustering step, we have several sub-graphs. In this step, we need to generate grid that fit each point as closely as possible. To represent the gird, we generate the base vector based on the orientation of every lines.
\par 
\par TODO: generate base vector for grid,  give the evaluation function etc.

\subsubsection{Fit Grid Point}
\par If the group satisfy the grid configuration, our next goal is to put each graph point into appropriate gird point. At the same time, satisfy the following criterial.
\begin{itemize}
	\item Each Beam(Bar,line) is a multiply of the length of a hole(20 lego unit).
	\item The shape should be as close as possible to the input user sketch.
\end{itemize}
\par Method: For each graph point, we generated 9 condidate closest point on grid. And try all the combination of all candidate point, find the feasible result which have the minimum score of the evaluation function.
\par Since we will try all the combinations of each point, so the calculation time is so important. The average number of nodes for a subgraph is 6, So the average trying numbers is $9^6$
\par Evaluation Function:We denote the $i_{th}$ point as $O_i$current candidate point on point $i$ as $P_i$. Then the evaluation function is $$\sum_{i=0}^{n-1}|Q_i-P_i|$$. After trying all combinations, the left thing is to find the result with minimal score.

\par TODO:give evaluation function(how close between the sketch and the assembly model), analyze the possible solution.

\subsubsection{Fit Non-Grid Point}
\par However, our user may not always give a grid-based input. So we should judge whether the graph satisfy the grid-shape configuration.
\par For Non-Grid graph, we also hold the two criterial above. But the Method are diffrent.
\par Method: Generate random point for each point in a roundness area. And expect each line become an multiply of 20.
\par If we just generate random number for each point, and expect them all satisfy the conditions at the same time. The possibility may be very small. So our algrithm choose to fit the point 3 by 3.

\subsubsection{Merge co-linear Beams}
\par For each point, we find its adjacent lines. And calculate whether two of them are co-linear, which means the two co-linear beams can be replaced by a long single beam.
THRESHOLD:
$$arcos(|\frac{\overrightarrow{l_1}\cdot\overrightarrow{l_2}}{|\overrightarrow{l_1}| \cdot |\overrightarrow{l_2}|}|)<\frac{\pi}{180}$$
\par TODO: give the evaluation function. And give adjustment strategy when it's slightly not co-linear.

\subsubsection{Layering Arrangement}
\par When we have the 2D graph in x-y plane, next stage is to generate the 2.5D model, which means layer each beam in z-direction.
\par We have the following criteria.
\begin{itemize}
	\item adjacent beams can not collide(at the same layer) \&\& can not be seperated.
	\item Minimize the number of layers.
\end{itemize}
Try all possible combinations, remove the symmetry configurations etc.

\par TODO: judgement algrithm, collision detection etc.


\par Notice: do not do Rigid analysis now, do it latere. Maybe not rigid for a single plane, but rigid for the whole structure.


\subsection{Plane Connection Algorithm}
Here will be an algorithm to use connect patterns to connect each plane, including changing the orientations of the beams.

Cite something for compilation...~\cite{song2016}


==> preprocess.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[!t]
  \centering
  \includegraphics[width=17cm]{images/optimize_SA.png}
  \vspace*{-2mm}
  \caption{Optimizing the local ``beam hole'' orientation, such that most adjacent beam holes have the same orientation for simple connections. \legoclaim}
%  \caption{Optimizing the local ``beam hole'' orientation, such that the number of adjacent beam holes with different orientations is minimized.}
%; note also the minimization of the objective value and the connected components in the optimized results.\phil{TODO: component}}
  \label{fig:optimize_SA}
  \vspace*{-2mm}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Preparing and Preprocessing the Input Design
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Two-Stage Framework: Stage 1}
\label{sec:our_framework1}

After the above modeling works, we are ready to arrange beams to construct Technic models and deal with the four sub-problems:
(i) which beams to use and where to put them;
(ii) the beam orientation;
(iii) the beam layering; and
(iv) the beam connections.

In our initial attempt, we explored various computational frameworks, e.g., beam search~\cite{wiki:Beam_search}, where we start from a random node in the guiding graph, arrange the first beam based on some heuristics,
%(e.g., start at low valence junctions), 
and progressively arrange locally-optimum beams to connect with previous ones.
%
Doing so produces coherently-connected models that cover the entire sketch, but the models are often badly optimized for model simplicity and structural integrity.
%
It is because beam search cannot effectively explore the global structure in the immense search space, except for simple models.
% since the problem incurs a particularly large solution space, beam search finds only locally good beam placement, thus the global structure and the overall solution are far from the optimum, except for simple models like the cube.
%
Besides beam search, we explored greedy set cover, ant colony search, and various metaheuristic strategies.
%
However, we found no success in efficiently finding near-optimum (or just feasible) results to fulfill the various requirements, especially for nontrivial inputs.

To this end, we formulate a {\em two-stage simulated-annealing-based framework\/}.
In stage one, we first estimate the local beam orientations (sub-problem (ii)) and identify connected coplanar components in the input sketch.
Then, in stage two, we arrange and connect beams over the guiding graph (sub-problems (i), (iii) \& (iv)) to generate a beam layout and iteratively refine it, as guided by the objective function.
%
In this section, we first present the first stage of the framework, and will present the second stage in Section~\ref{sec:our_framework2}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stage 1: Estimate Beam Orientation}
\label{ssec:beam_orient}
In LEGO Technic models, adjacent beams of the same orientation can be steadily connected by pins; see Figure~\ref{fig:gap_rigid}.
However, to build 3D models, we generally need to arrange beams in different orientations for building different parts in the models; see the corner in Figure~\ref{fig:example_conn_cover}.
%
Since the beam orientation strongly affects the overall structure and connections, we first estimate the local beam orientation over the guiding graph in the first stage of our framework.

\begin{wrapfigure}{r}{0.37\columnwidth}
	\vspace{-10pt}
	%\centering
	\hspace{-5pt}
	\includegraphics[width=0.36\columnwidth]{images/diff_orient.png}
	\hspace{-30pt}
	\vspace{-10pt}
\end{wrapfigure}
%
Mathematically, we represent a beam's orientation as a 3D vector that passes through the medial axis of the beam's holes; see the inset figure.
Particularly, we can flexibly rotate a beam about its associated line segment in the sketch (or equivalently, the edges that it covers in the guiding graph), as long as the beam's orientation vector is perpendicular to the line segment; see again the inset.
%
%as long as it is parallel to its associated line segment in the input sketch (see again the inset), meaning that we just require that the beam orientation vector is perpendicular to the beam's associated sketch line.
%
%when a beam is arranged to cover certain line segment in the input sketch, it should be parallel to the associated edge in the guiding graph (see again the inset), meaning that we just require that the beam orientation vector is perpendicular to the beam's associated sketch line.
%
%we can flexibly orientate a beam as long as it is parallel to its associated line segment in the input sketch (see again the inset), meaning that we just require that the beam orientation vector is perpendicular to the beam's associated sketch line.
%
Here, we model the problem of arranging beam orientation as an assignment problem.
Since most nodes in guiding graph $\mathcal{G}$ will eventually be covered by beams in the generated Technic model, we create a {\em hole orientation variable\/} for each node in $\mathcal{G}$.
%
Furthermore, since Technic bricks mostly lay on the principal (xy, yz and zx) planes, we should assign to each variable a principal direction (X, Y or Z), unless purposely specified in the user interface.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Objective.}
We aim to {\em minimize the number of adjacent node pairs with different hole orientations\/}, since adjacent nodes having the same orientations can be covered by a single beam that passes through them or by adjacent beams that are connected simply with pins.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Constraints}
%
(i) For non-junction nodes along line segments in the input sketch, their hole orientations should be perpendicular to the associated line segment~\footnote{\setlength{\columnsep}{3.5mm}
%
% wrapfigure margin
\begin{wrapfigure}{r}{0.27\columnwidth}
	\vspace{-20pt}
	%\centering
	\hspace{-5pt}
	\includegraphics[width=0.26\columnwidth]{images/single_hole.png}
	\hspace{-30pt}
	\vspace{-15pt}
\end{wrapfigure}
Except for short line segments with just a single interior hole (see the right inset figure), since we observe that in such situation, existing LEGO models may fill/cover the node using a single hole brick (near Figure~\ref{fig:brickset_and_connections} (top-left)) whose orientation aligns with the associated line segment.};
%\footnote{\setlength{\columnsep}{3.5mm} % wrapfigure margin
% (unless it is a single hole inbetween two endpoint junctions).
%
(ii) orientation of adjacent holes should be the same or perpendicular to each other; and
%, so that we may use a single beam to cover the two holes or connect them using the connection mechanisms shown in Figure~\ref{fig:brickset_and_connections} (right)
%
(iii) hole orientation variables at symmetry locations are constrained to be the same (for translational symmetry) or mirrored (for reflection symmetry).

\vspace*{-5pt}
\paragraph{Method.}
We solve this combinatorial optimization problem using a simulated annealing (SA) model~\cite{Wiki-2018-Simulated-Annealing}.
Initially, we randomize all hole orientation variables (see Figure~\ref{fig:optimize_SA} for examples) but following the listed constraints.
%
Then, we iteratively choose a random line segment, change the orientation of all the non-junction nodes in the segment, and update the orientation at each associated junction node, if the objective is minimized.
%
Figure~\ref{fig:optimize_SA} shows the initial state, optimized result, and objective values on three examples.
%
In our implementation, we set the initial temperature as $2\times10^3$, stopping temperature as $0.01$, and cooling rate as $1-\frac{10}{|\mathcal{V}|}$, where $\mathcal{V}$ is the node set in the guiding graph.
The optimization takes only a few seconds to complete for most models shown in the paper.
%
%Note also that if we run the method a few times, we may find multiple solutions of the same minimized objective value, e.g., {\sc cube}.
%In that case, we may try each solution independently in the second stage of our annealing framework.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[height=2.5cm]{images/plane_components.png}
\vspace*{-2mm}
\caption{The optimized {\sc airplane} in Figure~\ref{fig:optimize_SA} has 22 components. \legoclaim}
%, and we use the same color for each group of symmetric components.}
\label{fig:plane_components}
\vspace*{-2mm}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Find Components and Beam Placements}
\label{ssec:components}


%Component - a coplanar connected subgraph in the guiding graph whose nodes have the same orientation.

Next, we divide the nodes in guiding graph $\mathcal{G}$ into components, such that nodes in each component have the {\em same orientation\/} and are {\em coplanar\/}.
%
Here, $\mathcal{C}$ denotes the component set as in Eq.~\eqref{eq:cpt}.
%
For example, {\sc cube} and {\sc lifter} in Figure~\ref{fig:optimize_SA} have six and nine components, respectively, while {\sc airplane} has 22 components; see the exploded view in Figure~\ref{fig:plane_components}.
%
Moreover, we store symmetry information within and across components to facilitate subsequent computation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=7.8cm]{images/beam_placement.png}
\vspace*{-2mm}
\caption{Nine possible beam placements to cover the red edge. \legoclaim}
%\caption{There are nine possible beam placements that can cover the edge marked in red on the {\sc square} shape shown above.}
\label{fig:beam_placement}
\vspace*{-2mm}
\end{figure}


Furthermore, for each beam, we find the locations that we may place it on each component.
%
Hence, in each edge in a component, we can obtain {\em a list of feasible beam placements\/} that can cover the edge, and likewise, a list of beam placements that stop at or pass through each node; see Figure~\ref{fig:beam_placement}.
%
This data structure will help accelerate the layout generation in the second stage of our framework.









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\if 0
%
%This section will include:
%\begin{itemize}
%
%\item
%step 1: locate all the holes along the line segments
%
%\item
%step 2: SA - to optimize the hole orientation
%\begin{itemize}
%\item
%variable: each hole carries an orientation (X/Y/Z)
%\item
%constraints:
%  constraint 1: along a line segment, the hole orientation must be perpendicular to the line segment direction
%  constraint 2: non-endpt holes within a line segment must have the same orientation
%\item
%objective: minimize the total number of adjacent hole pairs whose orientations are different, with a 
%operation: randomly choose a line segment and change the orientation of all the non-endpt holes in the line segment, and then %update the orientation of each of the two endpt holes, such that the objective is minimized.
%\item 
%We use the basic SA model with parameters... TODO
%\end{itemize}
%
%\item
%step 3:
%symmetry in the first orientation estimation step:
%	lines in  positions have same orientation
%symmetry in the following construction process:
%	1) beams in the same 2D component
%	2) beams in different 2D components
%
%\item
%...
%
%\end{itemize}
%
%\fi
%

==> search.sig19.tex <==

\section{LEGO Technic Construction Search}
\label{sec:search}

Given a guiding graph, the search for a LEGO Technic construction involves four sub-problems:
(i) which beams to use and where to put them;
(ii) beam orientation;
(iii) beam layering; and
(iv) beam connections.
%
In our initial attempt, we tried various computational frameworks, e.g., beam search~\cite{wiki:Beam_search}, where we start from a random corner in the guiding graph,
%, arrange the first beam using heuristics, (e.g., start at low valence junctions), 
and progressively arrange locally-optimum beams.
%
Doing so produces coherently-connected models that cover the entire sketch, but the models are often poorly optimized for model simplicity and structural integrity.
It is because beam search cannot effectively explore the global structure in the immense search space.
%, except for simple models.
% since the problem incurs a particularly large solution space, beam search finds only locally good beam placement, thus the global structure and the overall solution are far from the optimum, except for simple models like the cube.
%
Besides, we explored greedy set cover, ant colony search, and various metaheuristic strategies.
%
However, we found no success in efficiently finding near-optimum results to fulfill the objectives, especially for nontrivial inputs.

To this end, we formulate a {\em two-stage simulated-annealing-based search framework\/}.
In stage one, we estimate the local beam orientations (sub-problem (ii)) and identify coplanar components in the input sketch.
In stage two, we initialize a random layout of beams over the guiding graph and iteratively refine it (sub-problems (i), (iii) \& (iv)), guided by the objective function $\mathcal{F}$.
%
%In this section, we first present the first stage of the framework, and will present the second stage in Section~\ref{sec:our_framework2}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=8.35cm]{images/beam_cover.pdf}
\vspace*{-2mm}
\caption{After we arrange the beams (left), we need to further arrange connection mechanisms (in orange) between adjacent beams (right). \legoclaim}
\label{fig:example_conn_cover}
\vspace*{-2mm}
\end{figure}

\begin{figure*}[!t]
  \centering
  \includegraphics[width=17cm]{images/optimize_SA.png}
  %\includegraphics[width=17cm]{images/optimize_SA.pdf}
  \vspace*{-2mm}
  \caption{Optimizing the ``beam hole'' orientations, such that most adjacent beam holes have the same orientation for simpler beam connections. \legoclaim}
%  \caption{Optimizing the local ``beam hole'' orientation, such that the number of adjacent beam holes with different orientations is minimized.}
%; note also the minimization of the objective value and the connected components in the optimized results.\phil{TODO: component}}
  \label{fig:optimize_SA}
  \vspace*{-1mm}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stage one: Estimating Beam Orientation}
\label{ssec:beam_orient}

In LEGO Technic models, adjacent beams of the same orientation can be steadily connected by pins.
%; see Figure~\ref{fig:gap_rigid}.
However, to build 3D models, we generally need to arrange beams in different orientations for building different parts of the models.
%; see the corner in Figure~\ref{fig:example_conn_cover}.
%
Since the beam orientation strongly affects the overall structure and connections, we first estimate the local beam orientation over the guiding graph.
%in the first stage of our framework.

\begin{wrapfigure}{r}{0.37\columnwidth}
	\vspace{-10pt}
	%\centering
	\hspace{-5pt}
	\includegraphics[width=0.36\columnwidth]{images/diff_orient.png}
	\hspace{-30pt}
	\vspace{-10pt}
\end{wrapfigure}
%
Mathematically, we represent a beam's orientation as a 3D vector that passes through the medial axis of the beam's holes; see the inset figure.
In general, we can reorient a beam, as long as the beam's orientation vector is perpendicular to its associated line segment in the sketch, or the edges that it covers in the guiding graph.
%
%as long as it is parallel to its associated line segment in the input sketch (see again the inset), meaning that we just require that the beam orientation vector is perpendicular to the beam's associated sketch line.
%
%when a beam is arranged to cover certain line segment in the input sketch, it should be parallel to the associated edge in the guiding graph (see again the inset), meaning that we just require that the beam orientation vector is perpendicular to the beam's associated sketch line.
%
%we can flexibly orientate a beam as long as it is parallel to its associated line segment in the input sketch (see again the inset), meaning that we just require that the beam orientation vector is perpendicular to the beam's associated sketch line.
%
Here, we model the problem of finding the beam orientation as an assignment problem.
Since most nodes in guiding graph $\mathcal{G}$ will eventually be covered by beams in the generated LEGO Technic model (the rest will be covered by connection mechanisms), we create a {\em hole orientation variable\/} for each node in $\mathcal{G}$.
%
Furthermore, since LEGO Technic bricks mostly lay on the principal (xy, yz and zx) planes, we should assign to each variable a principal direction (X, Y or Z), unless purposely specified in the user interface.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Objective.}
To {\em minimize the number of adjacent node pairs with different hole orientations\/} to encourage the use of pin and axle connections for model simplicity and structural integrity.
%since adjacent nodes having the same orientations can be covered by a single beam that passes through them or by adjacent beams that are connected simply using pins.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Constraints}
%
(i) For non-junction nodes along line segments in the input sketch, their hole orientations should be perpendicular to the associated line segment~\footnote{\setlength{\columnsep}{3.5mm}
%
% wrapfigure margin
\begin{wrapfigure}{r}{0.27\columnwidth}
	\vspace{-20pt}
	%\centering
	\hspace{-5pt}
	\includegraphics[width=0.26\columnwidth]{images/single_hole.png}
	\hspace{-30pt}
	\vspace{-15pt}
\end{wrapfigure}
Except for short line segments with just a single interior hole (see the right inset figure), since we observe that in such a situation, existing LEGO models may fill/cover the node using a single hole brick (near Figure~\ref{fig:brickset_and_connections} (top-left)) whose orientation aligns with the associated line segment.};
%\footnote{\setlength{\columnsep}{3.5mm} % wrapfigure margin
% (unless it is a single hole inbetween two endpoint junctions).
%
(ii) orientation of adjacent holes should be the same or perpendicular to each other, so that we may use a single beam to cover the two holes or connect them using a connection mechanism shown in Figure~\ref{fig:brickset_and_connections} (right); and
%
(iii) hole orientation variables at symmetry locations are constrained to be the same (for translational symmetry) or mirrored (for reflection symmetry).

%\vspace*{-5pt}
\paragraph{Method.}
We solve this combinatorial optimization problem using a simulated annealing (SA) model~\cite{Wiki-2018-Simulated-Annealing}.
Initially, we randomize all hole orientation variables (see Figure~\ref{fig:optimize_SA} for examples) but following the listed constraints.
%
Then, we iteratively choose a random line segment, change the orientation of all the non-junction nodes in the segment, and update the orientation at each associated junction node, if the objective is minimized.
%
Figure~\ref{fig:optimize_SA} shows the initial state, optimized result, and objective values for three examples.
%
In our implementation, we set the initial temperature as $2\times10^3$, stopping temperature as $0.01$, and cooling rate as $1-\frac{10}{|\mathcal{V}|}$, where $\mathcal{V}$ is the node set in the guiding graph.
The optimization takes only a few seconds to complete for most models shown in the paper.
%
%Note also that if we run the method a few times, we may find multiple solutions of the same minimized objective value, e.g., {\sc cube}.
%In that case, we may try each solution independently in the second stage of our annealing framework.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\linewidth]{images/beam_placement.png}
\vspace*{-2mm}
\caption{Nine possible beam placements to cover the red edge. \legoclaim}
%\caption{There are nine possible beam placements that can cover the edge marked in red on the {\sc square} shape shown above.}
\label{fig:beam_placement}
\vspace*{-2mm}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.9\linewidth]{images/plane_components.png}
\vspace*{-2mm}
\caption{The optimized {\sc airplane} in Figure~\ref{fig:optimize_SA} has 22 components. \legoclaim}
%, and we use the same color for each group of symmetric components.}
\label{fig:plane_components}
\vspace*{-2mm}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Find Components and Beam Placements}
%\label{ssec:components}


%Component - a coplanar connected subgraph in the guiding graph whose nodes have the same orientation.
\vspace*{-5pt}
\paragraph{Find ``components'' and ``beam placements''}
%
Next, we decompose the nodes in the guiding graph into components, such that nodes in each component have the {\em same orientation\/} and are {\em coplanar\/}.
%
%Here, $\mathcal{C}$ denotes the component set as in Eq.~\eqref{eq:cpt}.
%
For example, the optimized {\sc cube} and {\sc lifter} shown in Figure~\ref{fig:optimize_SA} have six and nine components, respectively, while the optimized {\sc airplane} has 22 components; see Figure~\ref{fig:plane_components}.
%
Also, we store symmetry information within and between components to facilitate computation.
%
Furthermore, for each beam, we find all locations that we may place it on each component.
%
Hence, for each edge in a component, we can obtain {\em a list of feasible beam placements\/} that can cover the edge, and likewise, a list of beam placements that stop at or pass through each node; see Figure~\ref{fig:beam_placement}.
%
This data structure will help accelerate the layout generation in the second stage of our framework.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[!t]
%  \centering
%  \includegraphics[width=8.35cm]{images/operator.png}
%  \vspace*{-1mm}
%  \caption{Operator to modify the beam layout.}
%%  \caption{The procedure in our operator to modify a beam layout; please see Section~\ref{ssec:update_operator} for the %procedural details.}
%  \label{fig:operator}
%  \vspace*{-2mm}
%\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[!t]
  \centering
  \includegraphics[width=8.35cm]{images/running_connection.png}
  \vspace*{-1mm}
  \caption{Steps to find connection mechanisms to join adjacent beams. \legoclaim}
%; see Section~\ref{ssec:connecting_beams} for the details.}
  \label{fig:running_connection}
  \vspace*{-2mm}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stage two: Beam Layout and Iterative Refinement}
\label{ssec:layout_refine}

Our annealing-based solution search in Stage 2 involves an iterative modification of a LEGO Technic construction for improving the objective function.
Here, the LEGO Technic construction starts as a layout of beams without connections, so we have to find optimal connection mechanisms to join adjacent beams in the layout to complete the construction; see Figure~\ref{fig:running_connection} for some examples.
Particularly, these connecting bricks (pins, axles, and connectors) should not collide with the existing beams nor with one another.
Also, they should not go below the ground plane in the 3D object space; please see supplemental material part E for the procedural details.

%The fundamental operations that are repeatedly applied include an operator which modifies the current beam layout and procedures to find connection mechanisms (see right of Figure~\ref{fig:brickset_and_connections}) to connect adjacent beams in a beam layout. In thesupplementary material, we provide details on the operator and beam connection, while the ensuing coverage focuses on the search process.

%\rz{Our annealing-based solution search in Stage 2 involves iterative modification of a LEGO Technic construction so as to improve the objective function.
%The fundamental operations that are repeatedly applied include an operator which modifies the current beam layout and procedures to 
%find connection mechanisms (see right of Figure~\ref{fig:brickset_and_connections}) to connect adjacent beams in a beam layout. In the
%supplementary material, we provide details on the operator and beam connection, while the ensuing coverage focuses on the search process.}

%Before presenting the overall search process, we in Section~\ref{ssec:main_procedure}, we first present how we modify a beam layout (Section~\ref{ssec:update_operator}) and connect adjacent beams (Section~\ref{ssec:connecting_beams}).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Layout initialization.}
Our solution search in Stage 2 starts by repeating the following two steps to initialize a beam layout:
%
(i) randomly pick an uncovered edge in the guiding graph (all edges are uncovered initially) and (ii) randomly select and add a feasible beam placement to cover the edge.
%, similar to steps (iii)-(v) in the layout modification operator (see Section~\ref{ssec:update_operator}).
%
%However, unlike the operator, 
Note that we select feasible beam placements with equal probability to deliberately generate a more random initial layout (see Figure~\ref{fig:overview}(c) for an example), since a more random layout helps the simulated annealing process avoid local minima.
%
% instead of greedily generating the initial layout to minimize the objective function, we deliberately generate a more random layout, so that the search process will not easily stuck at local minima.

%\phil{TODO: (i) how (the procedure to initialize) and (ii) discuss why this is sufficient already}
%Our initialization algorithm start from a guiding graph and an empty beam set $\mathcal{B}$.
%Then, the algorithm proceed as follows:
%\begin{itemize}
%	\item[(i)]
%	Randomly pick an uncovered edge $e$ in the guiding graph;
%	\item[(ii)] 
%	Find all possible beam placements that pass through edge $e$;
%	\item [(iii)]
%	We then randomly select a candidate beam $b$ with random layer number, add $b$ and its symmetry beams to $\mathcal{B}$; %and
%	\item [(iv)]
%	We repeat step (i), (ii), and (iii) until all the nodes in the guiding graph have a associate beam.
%\end{itemize}
%After the above procedure, we got $\mathcal{B}$ as a messy layout, see Figure. \ref{fig:overview} middle left for an initial %layout for our {\sc crossbow} model.
%%discussion
%Note that instead of creating a better initial layout using other strategies such as greedy, we deliberately add some random %variations to avoid the searching process start from a local minimum position, which may make the search process stuck in a local %region.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Layout modification operator.}
We design an effective operator to update the current beam layout.
By successively applying it, the search process can improve the beam layout with global modifications, while being able to converge at the end.
Before coming up with this design, we have explored many alternatives; see supplemental material part F for the operator procedure and discussion.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Objective function.}
As described in Algorithm~\ref{alg:SA}, we guide the beam layout refinement by minimizing the objective function $\mathcal{F}$, and use a simplified version denoted as $\mathcal{F}^0$ in the early annealing process for efficiency.
Adaptations of the objective for specific terms involving collision and connection coherence, as well as settings for all the parameters, can be found in supplementary material part D.

%\rz{We guide the beam layout refinement by minimizing the objective function $\mathcal{F}$, as described in Algorithm~\ref{alg:SA}.
%Adaptations of the objective function with respect to specific terms involving collison and connection coherence, as well as settings for all the parameters, can 
%be found in the supplementary material.}

%\phil{TODO:
%(i) we aim to minimize $\mathcal{F}$ (see Eq.~\eqref{eq:obj}) in order to create a beam layout for faithfulness to the input %sketch, structural simplicity, and structural integrity;
%(ii) weights on different terms in the objective functions... how to tune and why?
%(iii) for efficiency concern, we do not explicitly create beam connections (since the beam layout ...) over the annealing %process, some 
%then, define $\mathcal{F}^0$ and $\mathcal{F}^1$, which is the incomplete version and the complete version
%(iv) moreover, since the operator only modifies the local beam layout, we in fact locally update the objective function for %higher efficiency}

% minimization
%We optimize the beam layout by minimizing all the terms we mentioned in Section.\ref{sec:modeling}.
%% trade-off
%However, minimize one objective may violate another, so we can not achieve multiple optimal objective in a same beam layout. For %example, a simple layout which minimized the number of beam holes will contradict the rigidity objective, which need more than %one hole to for a rigid local connection.
%In Sec~\ref{sec:modeling}, most terms are served as penalty except for $\mathcal{F}_\text{dev}$ $\mathcal{F}_s$, and %$\mathcal{F}_\text{rgd}$.
%So impractically, we set $w2$,$w3$,$w6$,$w7$,$w8$ as $(?,?,?,?,?)$(check from code after I get back ), and leave the necessary %trade-off between $w_1$,$w_4$,$w_5$, and $w_9$ to user to indicate their preference.

% connectness evaluation -> slow
%Third, the algorithm to evaluation connection coherency in Eq.~\eqref{eq:cohr} contains procedure which require exhaustive search %for a local region, so it often takes more time than other terms. 
%Besides, we observe that at high temperatures, a simulated annealing algorithm accepts virtually all inferior steps and resembles %a random search, making the beams distribute sparsely and disordered. In this case, evaluating connectedness not much efficient %to guide the search, since nearly all the intermediate layout is not coherently connected.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% pseudo-code
\begin{algorithm}[!t] % enter the algorithm environment
\SetAlgoNoLine
\KwData{$T_\text{max}$, $T_\text{min}$, $T_\text{mid}$, $r$, and Guiding graph $\mathcal{G}$} 

$\mathcal{B}_\text{current} = \ \text{initialize}\_\text{layout}(\mathcal{G})$ \hspace*{3mm} \tcp{initialize the beam layout} 
$T \hspace*{6.95mm} = \ T_\text{max}$                                          \hspace*{20.25mm} \tcp{initialize temperature T}
$\mathcal{B}_\text{best} \hspace*{2.9mm} = \ \mathcal{B}_\text{current}$       \hspace*{16.75mm} \tcp{initialize the best layout}
$\mathcal{F}_\text{obj} \hspace*{4.05mm} = \ \mathcal{F}^o$                    \hspace*{21.75mm} \tcp{set objective func. in use}
\While{ \ $T \ > \ T_\text{min}$ \ }{
    \If{ \ $T \ < \ T_\text{mid}$ \ }{
        $\mathcal{F}_\text{obj} \ = \ \mathcal{F}$                             \hspace*{17.25mm} \tcp{switch to full obj. func.}
    }
	$\mathcal{B}_\text{new} = \ \text{modify}(\mathcal{B}_\text{current})$ \hspace*{4.75mm} \tcp{layout modification operator}
	$\Delta \ \hspace*{3.6mm} = \ \mathcal{F}_\text{obj}( \mathcal{B}_\text{new} ) \ - \ \mathcal{F}_\text{obj}( \mathcal{B}_\text{current} )$\;
	\If{\ $\exp(-\Delta / T ) \ > \ \text{rand}(0,1) $ \ }{
		$\mathcal{B}_\text{current} \ = \  \mathcal{B}_\text{new}$	\hspace*{21.75mm} \tcp{accept the change}
		\If{ \ $\mathcal{F}_\text{obj}(\mathcal{B}_\text{current}) \ > \ \mathcal{F}_\text{obj}(\mathcal{B}_\text{best}) $ \ }{
				$\mathcal{B}_\text{best} \ = \ \mathcal{B}_\text{current}$	\hspace*{17mm} \tcp{update best layout}
			}
	}
	$T \ = \ T*r$  \tcp*{update temperature $T$}
}
\textbf{return} \hspace*{1mm} $\mathcal{B}_\text{best}$
\caption{Procedure for iterative beam layout refinement} % give the algorithm a caption
\label{alg:SA} % and a label for \ref{} commands later in the document
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Overall procedure}
We adopt the simulated annealing model proposed by Cagan et al.~\shortcite{cagan1998simulated} to regulate the solution search process.
%
Our model has four parameters: $T_\text{max}$, $T_\text{mid}$, $T_\text{min}$ and $r$, which denote the starting temperature, middle cutoff temperature, ending temperature, and cooling rate, respectively.
We empirically set $T_\text{max}$ as $2$$\times$$10^3$, $T_\text{mid}$ as $10$, $T_\text{min}$ as $10^{-4}$, and $r$ (which trades off model quality and running time) as $0.999$ for simple models and as $0.99997$ for large complex models.
%
%In the annealing process, we use $\mathcal{F}^o$ when current temperature $T \geq T_\text{mid}$, and switch to use $\mathcal{F}$ when $T < T_\text{mid}$.
%
%Another important parameter is the cooling rate $r$ for trading off between the model quality and running time; we set $r$ as $0.999$ for simple models and as $0.99997$ for large and complex models.
%
Algorithm~\ref{alg:SA} presents the whole procedure.
%
%After initializing the beam layout and various parameters, we enter the main loop, which iteratively modifies the current beam layout $\mathcal{B}_\text{current}$ using the layout modification operator (denoted as modify()).
%
%In each iteration, we compute the change in the objective value (denoted as $\Delta$) after the layout modification, and accept the modification if $e^{-\Delta/T}$ is greater than a uniformly-distributed random value between zero and one, where $T$ is the current temperature in the annealing process.
%
%Lastly, when $T$ drops below $T_\text{min}$, the annealing process ends and returns the best beam layout $\mathcal{B}_\text{best}$ as the output.

%Recalling that we have four sub-problems when arranging beams to build Technic models.
%Among them, we first estimate the beam orientation based on a heuristic (see Section~\ref{ssec:beam_orient}), since addressing the four sub-problems altogether involves a tremendously large search space, which makes the overall problem hard to solve.
%
%However, we found that the estimated beam orientations may not be perfect all the time.
%Hence, when the beam layout become stabilized, we allow the layout modification operator to try different beam orientations (as long as the beam is still parallel to the associated sketch line) when adding beams, so that we may further improve the objective function.
%
%One typical example is the two pontoons on the bottom of the {\sc plane} model.
%The estimated orientation of the pontoon beams is upward (see Figure~\ref{fig:optimize_SA} (right)), but re-orientating the beams can allow simpler connection mechanisms (see Figure~\ref{fig:teaser}), thus further minimizing the objective function value.

%After the annealing procedure, output beams will have the same orientation with what we estimated in %Section.~\ref{ssec:beam_orient}.
%However, some line-shaped component may get a better connection by rotating along its central axis.
%To further improve, we try two different orthogonal orientation for each line-shaped component, and then choose one orientation %that could make simpler and coherent connection.
%%See the difference between the pink line-shaped component in bottom Figure~\ref{fig:plane_components} and the corresponding %position in the final model in Figure~\ref{fig:teaser} for example.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace*{-5pt}
\paragraph{Discussion}
%Recalling that we first estimate the beam orientation in Stage 1 of our framework; however, the estimated orientations may not be perfect all the time.
Since the beam orientations estimated in Stage 1 of our framework may not be perfect, we further allow the layout modification operator to try different valid beam orientations (see the constraints in Section~\ref{ssec:beam_orient}), when the beam layout becomes stable.
%
See Figure~\ref{fig:optimize_SA} (right) for the estimated orientation of the pontoon beams on the bottom of {\sc airplane}; re-orientating them allows simpler connections (see Figure~\ref{fig:teaser}) that minimize the objective.

Besides the exponential annealing schedule we adopted in our framework, we have tried several alternatives: linear, logarithmic, and optimum~\cite{nourani1998comparison}, as well as the thermodynamic schedule~\cite{de2003placement}.
However, we found no obvious improvements in the results and running time.
This is likely because the search space is discrete rather than continuous, where the feasible solutions are far from one another.
%
Also, we extended Algorithm~\ref{alg:SA} to be a population-based simulated annealing search~\cite{van2007population} by finding $N$ instead of one solutions in each iteration and keeping the best $K$ of them for generating the candidates in the next iteration (we set $N$ = 20 and $K$ = 4).
However, we found that the solution quality improves only slightly while the running time increases substantially, so we kept $N=K=1$ when producing our results.

%In addition, we have tried a population-based simulated annealing search method~\cite{van2007population}, where we first %independently initialize $N$ different random layouts, and in each iteration, pick the $k$ best layouts to continue their %executions, and restart the remaining $N-k$ layouts from the best solution found so far, where $N$ and $k$ are set as 20 and 4, %respectively.
%While the quality of the solutions improves slightly, the method requires much longer running time; see Section~\ref{sec:results} for comparison results.
%This proves our initialization algorithm provides a \phil{what do you mean by high?} starting searching point with high objective value, as a result, the search process do not easily to stuck in local minimum.

%Lastly, we have also tried metaheuristics and use a swamp to solve the problem.
%Particularly, we implemented an ant colony optimization method~\cite{dorigo1999ant}, where each move represents the addition of a new beam, so a model construction is represented by a sequence of moves started from an empty layout.
%
%Ideally, the optimization should converge to a near-shortest path, representing a simple beam layout, but we found the method can hardly converge to even a feasible layout, due to the exceptionally ``long path'' and huge search space incurred in the problem.
%\TODO{show experiments and real parameter setting}

% annealing schedule
%Ideally, a simulated annealing model can be further accelerated by carefully select a suitable annealing schedule.
%Except for exponential annealing schedule we used in our algorithm, we have attempted to implement several other predetermined %annealing schedules such as linear, logarithmic and optimum schedule as discussed in ~\cite{nourani1998comparison}, and adaptive %annealing schedule such at thermodynamic in ~\cite{de2003placement}. 
%However, the strategies did not improve the results nor the time. It is particularly challenging in the parameter setting, given %the fact that the search space is discrete and less connected.

% population
%Typically, due the fact that SA is a solo-searcher, its final solution quality may depends on the starting point.
%We experiment our algorithm stableness by implementing a population based SA search in ~\cite{van2007population}, where each %solution instances are initialized into different beam layout using our layout initialization algorithm.
%Since our initialization algorithm provides a high starting point, the search process can jump over hills to avoid stuck in local %minimum in the earlier process.
%As a result, the solution quality only improved slightly, while the running time is several times longer.
%See our experiments in Section. \ref{sec:result}(\TODO{show experiments}).

% swarm intellengence->, ant colony, particle swarm
%Another important family in metaheuristic algorithm is to use the behavior of swarms to solve the problem.
% ant colony
%We first implemented an ant colony optimization process, in which every move representing placing a new beam, and a set of moves %forms a path from empty beam set to a final construction.
%During the searching process, each ant will leave pheromone to indicate the shortest path(to a low-objective solution) they %found.
%Ideally, as time goes by, the pheromone content on the path leading to a low-objective solution will increase.
%However, the process can hardly converge to a feasible beam layout due to the very "long path" and vast variations from am empty %set to the final construction.

% particle swarm
% XH : TODO: try to complete here after the experiment

\input{postprocessing}


